Dust dynamics and evolution in expanding HII regions. I. Radiative drift of neutral and charged grains

We consider dust drift under the influence of stellar radiation pressure during the pressure-driven expansion of an HII region using the chemo-dynamical model MARION. Dust size distribution is represented by four dust types: conventional polycyclic aromatic hydrocarbons (PAHs), very small grains (VSGs), big grains (BGs) and also intermediate-sized grains (ISGs), which are larger than VSGs and smaller than BGs. The dust is assumed to move at terminal velocity determined locally from the balance between the radiation pressure and gas drag. As Coulomb drag is an important contribution to the overall gas drag, we evaluate a grain charge evolution within the HII region for each dust type. BGs are effectively swept out of the HII region. The spatial distribution of ISGs within the HII region has a double peak structure, with a smaller inner peak and a higher outer peak. PAHs and VSGs are mostly coupled to the gas. The mean charge of PAHs is close to zero, so they can become neutral from time to time because of charge fluctuations. These periods of neutrality occur often enough to cause the removal of PAHs from the very interior of the HII region. For VSGs, the effect of charge fluctuations is less pronounced but still significant. We conclude that accounting for charge dispersion is necessary to describe the dynamics of small grains.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%               Macros for TeX/LaTeX documents
%
% Author: Frank C. van den Bosch
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{{et al.~}}

\newcommand{\kmsmpc}{\>{\rm km}\,{\rm s}^{-1}\,{\rm Mpc}^{-1}}
%\newcommand{\kms}{\>{\rm km}\,{\rm s}^{-1}}
%\newcommand{\pc}{\>{\rm pc}}
\newcommand{\cm}{\>{\rm cm}}
\newcommand{\Mpc}{\>{\rm Mpc}}
\newcommand{\kpc}{\>{\rm kpc}}
\newcommand{\Msun}{\>{\rm M_{\odot}}}
\newcommand{\Lsun}{\>{\rm L_{\odot}}}
\newcommand{\MLsun}{\>({\rm M}/{\rm L})_{\odot}}
\newcommand{\Mbh}{M_{\bullet}}
\newcommand{\Vrot}{V_{\rm rot}}
\newcommand{\mtol}{\>{\rm (M/L)_{\odot}}}
\newcommand{\erg}{\>{\rm erg}}
\newcommand{\kpch}{\>{h^{-1}{\rm kpc}}}
\newcommand{\mpch}{\>h^{-1}{\rm {Mpc}}}
\newcommand{\yr}{\>{\rm yr}}
\newcommand{\yrs}{\>{\rm yrs}}
\newcommand{\Msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunh}{\>h^{-2}\rm L_\odot}
\newcommand{\calN}{{\cal N}}
\newcommand{\wcalN}{\tilde{{\cal N}}}
\newcommand{\walpha}{\tilde{\alpha}}
\newcommand{\wLstar}{\tilde{L}^{*}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\lamA}{${\Lambda}30/90 \, $}
\newcommand{\lamC}{${\Lambda}25/75 \, $}
\newcommand{\lamD}{${\Lambda}20/65 \, $}
\newcommand{\lamB}{${\Lambda}30/65 \, $}
\newcommand{\reference}{\bibitem}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\vcir}{V_{\rm c}}
\newcommand{\vh}{V_{\rm c}}
\newcommand{\Obaryon}{{\Omega_{\rm B,0}}}
\newcommand{\Kdegree}{\>{\rm K}}
\newcommand{\keV}{\>{\rm keV}}
\newcommand{\vhalo}{V_{\rm c}}
\newcommand{\Tvir}{T_{\rm vir}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\vesc}{V_{\rm esc}}
\newcommand{\Lya}{{\rm Ly}\alpha}
\newcommand{\msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunhh}{\,h^{-2}\rm L_\odot}
\newcommand{\Msunhh}{\,h^{-2}\rm M_\odot}

%%% 
\newcommand{\lcen}{L}
\newcommand{\msc}{M_{\rm *c}}
\newcommand{\pc}{Q}
\newcommand{\pten}{Q_{\rm 10}}
\newcommand{\lc}{\lcen}
\newcommand{\avg}[1]{\langle #1 \rangle}
\newcommand{\avglogm}{\avg{\log M}(\lcen)}
\newcommand{\avglogmsq}{\avg{(\log M)^2}(L_c)}
\newcommand{\avgloglc}{\avg{\log \lcen}(M)}
\newcommand{\siglogm}{\sigma_{\log M}(\lcen)}
\newcommand{\ploglcm}{P(\log \lcen|M)}
\newcommand{\plogmlc}{P(\log M|\lcen)}
\newcommand{\drm}{{\rm d}}
\newcommand{\pdv}{{P (\Delta V)}}
\newcommand{\dv}{{\Delta V}}
% \newcommand{\sigcen}{\sigma_{\rm cen}}
\newcommand{\siglcen}{\sigma_{\log L}}
\newcommand{\sigcenm}{\sigma_{\log M_*}}
\newcommand{\sigmscen}{\sigma_{\log M_*}}
\newcommand{\sigp}{\sigma_{\log Q}}
\newcommand{\sigcenp}{\sigma_{\log Q}}
\newcommand{\sigsw}{\sigma_{\rm sw}}
\newcommand{\sighw}{\sigma_{\rm hw}}
\newcommand{\sigsat}{\sigma_{\rm sat}}
\newcommand{\avgsigsatsq}{\avg{\sigsat^2}}
\newcommand{\avnsat}{\avg{N_{\rm s}}}
\newcommand{\avnsatm}{\avnsat(M)}
\newcommand{\philcm}{\Phi_{\rm c}(L|M)}
\newcommand{\philsm}{\Phi_{\rm s}(L|M)}
\newcommand{\plcm}{P(\lcen|M)}
\newcommand{\pmscm}{P(\msc|M)}
\newcommand{\pmlc}{P(M|\lcen)}
\newcommand{\pmpc}{P(M|\pc)}
\newcommand{\ppcm}{P(\pc|M)}
\newcommand{\sigav}{\sigma_{\rm av}}
%special
\newcommand{\fr}{f_{\rm r}}
\newcommand{\fb}{f_{\rm b}}
\newcommand{\fint}{f_{\rm int}}
\newcommand{\sigr}{\sigma_{\rm r}}
\newcommand{\sigb}{\sigma_{\rm b}}
\newcommand{\Mr}{M_{\rm r}}
\newcommand{\Mb}{M_{\rm b}}
\newcommand{\Rh}{R_{\rm h}}
\newcommand{\Rs}{R_{\rm s}}
\newcommand{\dvh}{(\dv)_{\rm h}}
\newcommand{\dvs}{(\dv)_{\rm s}}
\newcommand{\Sset}{\hat{S}}
%%%%% less than approximate and all that

\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\prosima{$\; \buildrel \propto \over \sim \;$}
\def\gsim{\lower.7ex\hbox{\gtsima}}
\def\lsim{\lower.7ex\hbox{\ltsima}}
\def\simgt{\lower.7ex\hbox{\gtsima}}
\def\simlt{\lower.7ex\hbox{\ltsima}}
\def\simpr{\lower.7ex\hbox{\prosima}}
\def\la{\lsim}
\def\ga{\gsim}
\def\lta{\la}
\def\gta{\ga}

%%%%%% Useful for editing drafts

\newcommand{\XXX}[2]{{\sf #1}}
\newcommand{\QQQ}[1]{{\sc $<$#1$>$}}

%To return to the original version, comment the previous two lines and
%uncomment the next two lines 

%\newcommand{\XXX}[2]{#2}
%\newcommand{\QQQ}[1]{}

%%%%%% Useful for bibliography

\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJL}
\newcommand{\apjs}{ApJS}
\newcommand{\aj}{AJ}
\newcommand{\mnras}{MNRAS}
\newcommand{\aap}{A\&A}
\newcommand{\aaps}{A\&AS}
\newcommand{\araa}{ARA\&A}
\newcommand{\nat}{Nature}
\newcommand{\pasp}{PASP}

%%%%%% Useful measures of length for use with psfig

\newdimen\hssize
\hssize=8.4truecm
\newdimen\hdsize
\hdsize=17.7truecm

%%%%%%

\def\fn#1{$^{\ref{#1}}$}
\def\fit#1{\footnotesize \it #1 }
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

